Model Inversion Networks for Model-Based Optimization

In this work, we aim to solve data-driven optimization problems, where the goal is to find an input that maximizes an unknown score function given access to a dataset of inputs with corresponding scores. When the inputs are high-dimensional and valid inputs constitute a small subset of this space (e.g., valid protein sequences or valid natural images), such model-based optimization problems become exceptionally difficult, since the optimizer must avoid out-of-distribution and invalid inputs. We propose to address such problem with model inversion networks (MINs), which learn an inverse mapping from scores to inputs. MINs can scale to high-dimensional input spaces and leverage offline logged data for both contextual and non-contextual optimization problems. MINs can also handle both purely offline data sources and active data collection. We evaluate MINs on tasks from the Bayesian optimization literature, high-dimensional model-based optimization problems over images and protein designs, and contextual bandit optimization from logged data.

==> Model inversion networks (MINs)/defs.tex <==
%% editing comment
\newcommand{\cmt}[1]{{\textcolor{red}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\todo}[1]{\cmt{TO-DO: #1}}
\newcommand{\cmtt}[1]{{\textcolor{blue}{#1}}}


%% abbreviations
\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\etal}{{et~al.}\ }
\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }
\newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\trace}{\text{tr}}

%% specifics for the paper
\newcommand{\reward}{r}
\newcommand{\policy}{\pi}
\newcommand{\mdp}{\mathcal{M}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\observations}{\mathcal{O}}
\newcommand{\transitions}{\mathcal{T}}
\newcommand{\initial}{\mathcal{I}}
\newcommand{\horizon}{H}
\newcommand{\rewardevent}{R}
\newcommand{\probr}{p_\rewardevent}
\newcommand{\metareward}{\bar{\reward}}

\newcommand{\pihi}{\pi^{\text{hi}}}
\newcommand{\pilo}{\pi^{\text{lo}}}
\newcommand{\ah}{\mathbf{w}}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\eye}{\mathbf{I}}

\newcommand{\model}{\hat{p}}

\newcommand{\pimix}{\pi_{\text{mix}}}

\newcommand{\pib}{\bar{\pi}}
\newcommand{\epspi}{\epsilon_{\pi}}
\newcommand{\epsmodel}{\epsilon_{m}}

%% math
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\en}{\mathcal{E}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\ot}{\bo_t}
\newcommand{\st}{\bs_t}
\newcommand{\at}{\ba_t}
\newcommand{\op}{\mathcal{O}}
\newcommand{\opt}{\op_t}
\newcommand{\kl}{D_\text{KL}}
\newcommand{\tv}{D_\text{TV}}
\newcommand{\ent}{\mathcal{H}}
\newcommand{\actionspace}{\mathcal{A}}
\newcommand{\filt}{\mathcal{F}}
\newcommand{\expec}{\mathbb{E}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\piinv}{\pi^{-1}}
\newcommand{\finv}{f^{-1}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\atcn}{A_t^{\mathrm{CN}}}
\newcommand{\atts}{A_t^{\mathrm{TS}}}
\newcommand{\bzhi}{\bz^\text{hi}}
\newcommand{\inputspace}{\mathcal{X}}
\newcommand{\yquery}{\tilde{y}^*}
\newcommand{\zquery}{\tilde{z}^*}
\newcommand{\disc}{\operatorname{Disc}}
\newcommand{\jsd}{D_{\text{JSD}}}

\newcommand{\question}[1]{\cmt{\textbf{Question}: #1}}
\newcommand{\sergey}[1]{\cmt{#1}}
\newcommand{\aviral}[1]{\cmt{#1}}
\newcommand{\aviralnew}[1]{\cmtt{#1}}



==> Model inversion networks (MINs)/experiments.tex <==
\section{Experimental Evaluation}
\label{sec:experiments}

The goal of our empirical evaluation is to answer the following questions. \textbf{(1)} Can MINs successfully solve optimization problems of the form shown in Equations~(\ref{eq:optimization}) and (\ref{eq:contextual_optimization}), in static settings and active settings, better than or comparably to prior methods?
\textbf{(2)} Can MINs generalize to high dimensional spaces, where valid inputs $\x$ lie on a lower-dimensional manifold, such as the space of natural images? \textbf{(3)} Is reweighting the data distribution important for effective data-driven model-based optimization? \textbf{(4)} Does our proposed inference procedure effectively discover valid inputs $\x$ with better values than any value seen in the dataset? \textbf{(5)} Does randomized labeling help in active data collection?

\subsection{Data-Driven Optimization with Static Datasets}
We first study the \emph{data-driven} model-based optimization setting. This requires generating points that achieve a better score than any point in the training set or, in the contextual setting, better than the policy that generated the dataset \emph{for each context}. We evaluate our method on a batch contextual bandit task proposed in prior work~\citep{joachims2018deep}, and on a high-dimensional contextual image optimization task. We also evaluate our method on several non-contextual tasks that require optimizing over high-dimensional image inputs to evaluate a semantic score function, including hand-written characters and real-world photographs.

\textbf{Batch contextual bandits.} We first study the contextual optimization problem described in Equation~(\ref{eq:contextual_optimization}).
{The goal is to learn a policy, purely from static data, that predicts the correct bandit arm $\x$ for each context $c$, such that the policy achieves a high score $f(c, \pi(c))$ on average across contexts drawn from a distribution $p(c)$.}  We follow the protocol set out by \citet{joachims2018deep}, which evaluates contextual bandit policies trained on a static dataset for a simulated classification tasks. The data is constructed by selecting images from the {(MNIST/CIFAR)} dataset as the context {$c$}, a random label as the \emph{input} {$\x$}, and a binary indicator indicating whether or not the label is correct as the \emph{score} {$y$}. {Multiple schemes can be used for mapping contexts to labels for generating the training dataset, and we evaluate on two such schemes, as described below. We report the average score on a set of new contexts, which is equal to the average 0-1 accuracy of the learned model on a held out test set of images (contexts).} We compare our method to previously proposed techniques, including the BanditNet model proposed by \citet{joachims2018deep} on the MNIST and CIFAR-10~\citep{Krizhevsky09learningmultiple} datasets. Note that this task is different from regular classification, in that the observed feedback ($(c_i, \x_i, y_i)$ pairs) is partial, i.e. we do not observe the correct label for each context (image) $c_i$, but only whether or not the label in the training tuple is correct or not.
\begin{table*}[t]
\centering 
\begin{tabular}{|l|r|r|r|r|r|}
\hline
\textbf{Dataset \& Type} & \textbf{BanditNet} & \textbf{BanditNet$^*$} & \textbf{MIN w/o I} & \textbf{MIN (Ours)} & \textbf{MINs w/o R} \\ \hline
MNIST ($49\%$ corr.) & $36.42 \pm 0.6$ & $-$ & $94.2 \pm 0.13$ & \textbf{95.0 $\pm$ 0.16} & 95.0 $\pm$ 0.21 \\
MNIST (Uniform) & $9.94 \pm 0.0 $& $-$ & $92.21 \pm 0.22$ & \textbf{93.67 $\pm$ 0.51} & 92.8 $\pm$ 0.01  \\
\hline
CIFAR-10 ($49\%$ corr.) & $42.13 \pm  2.35$ &  $87.0$ & $91.35 \pm 0.87$ & \textbf{92.21 $\pm$ 1.0} & 89.02 $\pm$ 0.05 \\
CIFAR-10 (Uniform) & $14.43 \pm 1.43$ & $-$ & $76.31 \pm 0.40$ & \textbf{77.12 $\pm$ 0.54} & 74.87 $\pm$ 0.12 \\
\hline
\end{tabular}
\caption{Test accuracy on MNIST and CIFAR-10 with 50k bandit feedback training examples. BanditNet$^*$ is the result from \citet{joachims2018deep}, while the BanditNet column is our implementation; we were unable to replicate the performance from prior work (details in Appendix~\ref{app:details}). MINs outperform both BanditNet and BanditNet$^*$, both with and without the inference procedure in Section~\ref{sec:inference}. {MINs w/o reweighting perform at par with full MINs on MNIST, and slightly worse on CIFAR 10, while still outperforming the baseline.}}
\label{table:bandit_perf}
\end{table*}
We evaluate on two datasets: (1) data generated by selecting random labels $\x_i$ for each context $c_i$ and (2) data where the correct label is used 49\% of the time, which matches the protocol in prior work~\citep{joachims2018deep}.
We compare to BanditNet~\citep{joachims2018deep} on identical dataset splits. We report the average 0-1 test accuracy for all methods in Table~\ref{table:bandit_perf}. The results show that MINs drastically outperform BanditNet on both MNIST and CIFAR-10 datasets, indicating that MINs can successfully perform contextual model-based optimization in the static (data-driven) setting.

{\textbf{Ablations.} The results in Table~\ref{table:bandit_perf} also show that utilizing the inference procedure in Section~\ref{sec:inference} produces an improvement of about 1.5\% and 1.0\% in test-accuracy on MNIST and CIFAR-10, respectively. Utilizing reweighting gives a slight performance boost of about 2.5\% on CIFAR-10.}

\begin{figure*}[t!]
\vspace{-10pt}
\centering
    \begin{subfigure}[t]{0.28\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth]{images/mnist_optimization_fig1.png}
        % \vspace{-0.12in}
        \includegraphics[width=0.9\linewidth]{images/mnist_optimization.png}
        \caption{Thickest stroke}
    \end{subfigure}%
    \begin{subfigure}[t]{0.27\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth]{images/mnist_optimization_fig2.png}
        % \vspace{-0.1in}
        \includegraphics[width=0.9\linewidth]{images/mnist_optimization_1.png}
        \caption{Thickest digit (3)}
    \end{subfigure}
    \begin{subfigure}[t]{0.27\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{images/mnist_optimization_fig3.png}
        % \vspace{-0.1in}
        \includegraphics[width=0.9\linewidth]{images/mnist_optimization_2.png}
        \caption{Most number of blobs (8)}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Results for non-contextual static dataset optimization on MNIST: (a) and (b): Stroke width optimization, and (c): Maximization of disconnected black pixel blobs. From left to right: MINs, MINs w/o Inference (Section~\ref{sec:inference}), {which sample $\x$ from the inverse map conditioned on the highest seen value of $y$}, MINs w/o Reweighting (Section~\ref{sec:reweighting}), and direct optimization of a forward model, {which starts with a random image from the dataset and updates it via stochastic gradient descent for the highest score based on the forward model.} Observe that MINs can produce thickest characters which resemble valid digits. Optimizing the forward function often turns non-digit pixels on, thus going off the valid manifold. Both the reweighting and inference procedure are important for good results. {Scores are mentioned beneath each figure. The larger score the better, provided the solution $\x$ is the image of a \textit{valid} digit.} Dataset average is \textbf{149.0}.}
    \label{fig:mnist_non_contextual}
    \vspace{-10pt}
\end{figure*}

\textbf{Character stroke width optimization.}
In the next experiment, we study how well MINs optimize over high-dimensional inputs, where valid inputs lie on a lower-dimensional manifold. We constructed an image optimization task out of the MNIST~\citep{lecun2010mnisthandwrittendigit} dataset. The goal is to optimize \textit{directly} over the image pixels, to produce images with the thickest stroke width, {such that the image corresponds, in the first scenario, (a) -- to any valid character, and in the second scenario, (b), to a valid instance of a particular character class ($3$ in this case).} A successful algorithm will produce the thickest character that is still recognizable. 

In Figure~\ref{fig:mnist_non_contextual}, we observe that MINs generate images $\x$ that maximize the respective score functions in each case. We also evaluate on a harder task, where the goal is to maximize the number of disconnected blobs of black pixels in an image of a digit. For comparison, we evaluate a method that directly optimizes the image pixels with respect to a forward model, of the form ${f}_\theta(\x)$. In this case, the solutions are far off the manifold of valid characters. 

{\textbf{Ablations.} We also compare to MINs without reweighting (MIN-R) and without the inference procedure (MIN-I), where $y$ is the maximum possible $y$ in the dataset to demonstrate the benefits of these two aspects. Observe that MIN-I sometimes yeilds invalid solutions ((a) and (c)), and MIN-R fails to output $\x$ belonging to the highest score class ((a) and (c)), thus indicating their importance.}

\textbf{Semantic image optimization.}
The goal in these tasks is to quantify the ability of MINs to optimize high-level properties that require semantic understanding of images. We consider MBO tasks on the IMDB-Wiki faces~\citep{Rothe2015DEX, Rothe2016Deep} dataset, where the function $f(\x)$ is the negative of the age of the person in the image. Hence, images with younger people have higher scores.
\begin{figure*}[t]
\begin{subfigure}[t]{1.0\textwidth}
    \vspace{-10pt}
        \centering
        \includegraphics[width=0.8\linewidth]{images/imdb_non_contextual/imdb_groundtruth_annotated.png}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_3_15_new.png}
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_1_15_new.png}
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_4_15_new.png}
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_2_15_new.png}
    \caption{Optimized $\x$ (trained on > 15 years)}
\end{subfigure}
~
\begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_1_25.png}
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_2_25.png}
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_3_25.png}
    \includegraphics[width=0.24\linewidth]{images/imdb_non_contextual_annotated/sample_4_25.png}
    \caption{Optimized $\x$ (trained on > 25 years)}
\end{subfigure}%
    \caption{MIN optimization to obtain the youngest faces ($\x$) when trained on faces older than 15 (left) and older than 25 (right). {The score function being optimized (maximized) in this case is the negative age of the face.} Generated optimization output $\x$ (bottom) are obtained via inference in the inverse map at different points during model training. Real faces ($\x$) of varying ages (including ages lower than those used to train the model) are shown in the top rows. We overlay the actual negative score (age) for each face on the real images, and the age obtained from subjective user rankings on the generated faces.} 
    \label{fig:non_contextual_imdb}
    \vspace{-10pt}
\end{figure*}

We construct two versions of this task: one where the training data consists of all faces older than 15 years, and the other where the model is trained on all faces older than 25 years. This ensures that our model cannot simply copy the youngest face. To obtain ground truth scores for the generated faces, we use subjective judgement from human participants. We perform a study with 13 users. Each user was asked to answer a set of 35 binary-choice questions each asking the user to pick the older image of the two provided alternatives. We then fit an age function to this set of binary preferences, analogously to \citet{Christiano2017DeepRL}.

\begin{wraptable}{l}{4.0cm}
\vspace{-10pt}
{\centering
\caption{Quantitative score-values for Youngest Face Optimization Task (larger the better)}
\label{table:face_opt_new}
\vspace{-15pt}
{\small
\begin{tabular}{lrr}\\\toprule
\textbf{Task} & \textbf{MIN} & \textbf{MIN (best)} \\\midrule
\emph{$\geq$ 15} & \textbf{-13.6} & -12.2 \\ \midrule
\emph{$\geq$ 25} & \textbf{-26.2} & -23.9 \\  \bottomrule
\end{tabular}}
\vspace{-10pt}
}
\end{wraptable}
Figure~\ref{fig:non_contextual_imdb} shows the images produced by MINs. For comparison, we also present some sample of images from the dataset partitioned by the ground truth score. We find that the most likely age for optimal images produced by training MINs on images of people 15 years or older was \textbf{13.6 years}, with the best image having an age of \textbf{12.2}. The model trained on ages 25 and above produced more mixed results, with an average age of \textbf{26.2}, and a minimum age of \textbf{23.9}. {We report these results in Table~\ref{table:face_opt_new}.} This task is exceptionally difficult, since the model must extrapolate outside of the ages seen in the training set, picking up on patterns in the images that can be used to produce faces that appear \emph{younger} than any face that the model had seen, while avoiding unrealistic images.


We also conducted experiments on \emph{contextual} image optimization with MINs.
We studied contextual optimization over hand-written digits to maximize stroke width, using either the character category as the context $c$, or the top one-fourth or top half of the image. In the latter case, MINs must learn to complete the image while maximizing for the stroke width. In the case of class-conditioned optimization, MINs attain an average score over the classes of \textbf{237.6}, while the dataset average is \textbf{149.0}.
\begin{wraptable}{r}{4.5cm}
\vspace{-10pt}
{\centering
\caption{Quantitative score values for MNIST inpainting (contextual)}
\label{table:inpaint_new}
\vspace{-15pt}
{\small
\begin{tabular}{lrr}\\\toprule
\textbf{Mask} & \textbf{MIN} & \textbf{Dataset} \\\midrule
\emph{mask A} & \textbf{223.57}  & 149.0 \\ \midrule
\emph{mask B} & \textbf{234.32} & 149.0 \\  \bottomrule
\end{tabular}}
\vspace{-10pt}
}
\end{wraptable}
In the case where the context is the top half or quarter of the image, MINs obtain average scores of \textbf{223.57} and \textbf{234.32}, respectively, while the dataset average is \textbf{149.0} for both tasks. {We report these results in Table~\ref{table:inpaint_new}.} We also conducted a contextual optimization experiment on faces from the Celeb-A dataset, with some example images shown in Figure~\ref{fig:celeba_contextual}. The context corresponds to the choice for the attributes brown hair, black hair, bangs, or moustache. The optimization score is given by the sum of the attributes wavy hair, eyeglasses, smiling, and no beard. Qualitatively, we can see that MINs successfully optimize the score while obeying the target context, though evaluating the true score is impossible without subjective judgement on this task. We discuss these experiments in more detail in Appendix~\ref{app:contextual}.
\vspace{-5pt}
\subsection{Optimization with Active Data Collection}
In the active MBO setting, MINs must select which \emph{new} datapoints to query to improve their estimate of the optimal input. In this setting, we compare to prior model-based optimization methods, and evaluate the exploration technique described in Section~\ref{sec:exploration}.
\begin{wrapfigure}{r}{4.5cm}
    \centering
    \vspace{-15pt}
        \includegraphics[width=1.0\linewidth]{images/contextual_images_celeba_main.png}
        \caption{{\small Optimized $\x$ produced from contextual training on Celeb-A. Context = (brown hair, black hair, bangs, moustache and $f(\x) = \ell_1$(wavy hair, eyeglasses, smiling, no beard). We show the produced $\x^\star$ for two contexts. The model optimizes score for both observed contexts such as brown or black hair and extrapolates to unobserved contexts such as brown and black hair.}}
        \vspace{-15pt}
    \label{fig:celeba_contextual}
\end{wrapfigure}

\textbf{Global optimization on benchmark functions.} We first compare MINs to prior work in Bayesian optimization on
standard benchmark problems (DNGO)~\citep{snoek15scalable}: the 2D Branin function, and the 6D Hartmann function.
As shown in Table~\ref{table:gp_tasks}, MINs reach within $\pm 0.1$ units of the global \textit{minimum} (minimization is performed here, instead of maximization), performing comparably with commonly used Bayesian optimization methods based on Gaussian processes. We do not expect MINs to be as efficient as GP-based methods, since MINs rely on training parametric neural networks with many parameters, which is less efficient than GPs on low-dimensional tasks.
Exact Gaussian processes and adaptive Bayesian linear regression~\citep{snoek15scalable} outperform MINs in terms of optimization precision and the number of samples queried, but MINs achieve comparable performance with about $4\times$ more samples. 

{\textbf{Ablations.} We also report the performance of MINs without the random labeling query method, instead selecting the next query point by greedily maximizing the current model with some additive noise (MIN + greedy). Random labeling method produces better results than the greedy data collection approach, indicating the importance of effective active data collection methods for MINs.}
\begin{table*}[t]
    \centering
    \footnotesize{
    \begin{tabular}{|l|r|r|r|r|}
        \hline
        \textbf{Function} & \textbf{Spearmint} & \textbf{DNGO} & \textbf{MIN} & \textbf{MIN + greedy}\\ \hline
        Branin (0.398) & $0.398 \pm 0.0$ & $0.398 \pm 0.0$  & $0.398 \pm 0.02$ & $0.4 \pm 0.05$(800) \\
        Hartmann6 (-3.322) & $-3.3166 \pm 0.02$ & $-3.319 \pm 0.00$ & $-3.315 \pm 0.05$(600) & $-3.092 \pm 0.12$(1200) \\
        \hline
    \end{tabular}
    }
    \caption{Active MBO on benchmark functions. The prior methods converge within 200 iterations. MINs require more iterations on some of the tasks, in which case we indicate the number of iterations in brackets. MINs reach similar final performance, and typically require 1-4$\times$ as much data as efficient GP-based algorithms.}
    \label{table:gp_tasks}
\end{table*}

% \vspace{-10pt}
\textbf{Protein fluorescence maximization.} In the next experiment, we study a high-dimensional active MBO task, previously studied by \citet{brookes19a}. This task requires optimizing over protein designs by selecting variable length sequences of codons, where each codon can take on one of 20 values. {In order to model discrete values, we use a Gumbel-softmax GAN also previously employed in~\citep{Gupta2018FeedbackG}, and as a baseline in~\citep{brookes19a}. For backpropagation, we choose a temperature $\tau=0.75$ for the Gumbel-softmax operation. This is also mentioned in Appendix \ref{app:details}.} The aim in this task is to produce a protein with maximum fluorescence. Each algorithm is provided with a starting dataset, and then allowed a identical, limited number of score function queries. {For each query made by an algorithm, it receives a score value from an oracle. We use the trained oracles released by \cite{brookes19a}. These oracles are separately trained forward models, and are inaccurate, especially for datapoints not observed in the starting static dataset.}

We compare to CbAS~\citep{brookes19a} and other baselines, including CEM {(cross entropy method)}, RWR {(reward weighted regression)} and {a method that uses a forward model -- GB~\citep{GmezBombarelli2018AutomaticCD} reported by \citet{brookes19a}}. 
\begin{wraptable}{r}{4.5cm}
\vspace{-15pt}
\footnotesize{
\begin{tabular}{lrr}\\\toprule
\textbf{Method} & \textbf{Max} & \textbf{50$\%$ile} \\ \midrule
\emph{\textbf{MIN (Ours)}} & \textbf{3.42}  & 3.24 \\ 
\emph{MIN - R} & 3.37 & \textbf{3.28} \\
\emph{CbAS} & {3.36} & \textbf{3.28} \\  
\emph{RWR} & $\sim$ 3.00 & $\sim$ 2.97 \\ 
\emph{CEM-PI} & $\sim$ 2.92& $\sim$ 2.9 \\ 
\emph{GB$^*$} & $\sim$ 3.25 & $\sim$3.25 \\ \bottomrule
\end{tabular}
}
\caption{Protein design results, with maximum fluorescence and the 50$^\text{th}$ percentile out of 100 samples. Prior method results are from \citet{brookes19a}. MINs perform comparably to CbAS. MINs without reweighting (MIN-R) lead to more consistent sample quality (higher 50$\%$ile score), while MINs with reweighting can produce the highest scoring sample.}
\label{table:protein}
\vspace{-10pt}
\end{wraptable}
{For evaluation, we report the ground truth score of the output of optimization (max), and the 50th-percentile ground truth score of all the samples produced via sampling (without inference, in case of MINs) so as to be comparable to \cite{brookes19a}.} In Table~\ref{table:protein}, we show that MINs are comparable to the best performing method on this task, and produce samples with the highest score among all the methods considered.

{\textbf{Ablations.} In Table~\ref{table:protein}, we also compare to MINs without reweighting in the active setting, which lead to more consistent sample quality (higher 50\% score), but do not produce the highest scoring sample unlike MINs with reweighting.} 

These results suggest that MINs can perform competitively with previously proposed model-based optimization methods in the active setting, reaching comparable or better performance when compared both to Bayesian optimization methods and previously proposed methods for a higher-dimensional protein design task.


==> Model inversion networks (MINs)/intro.tex <==
\section{Introduction}

Data-driven optimization problems arise in a range of domains: from protein design~\citep{brookes19a} to automated aircraft design~\citep{hoburg2012}, from the design of robots~\citep{liao2019} to the design of neural network architectures~\citep{zoph2017}. Such problems require optimizing unknown score functions using datasets of input-score pairs, without direct access to the score function being optimized. This can be especially challenging when valid inputs lie on a low-dimensional manifold in the space of all inputs, e.g., the space of valid aircraft designs or valid images. Existing methods to solve such problems often use derivative-free optimization~\citep{snoek2012practical}. Most of these techniques require \emph{active} data collection, where the unknown function is queried at new inputs. However, when function evaluation involves a complex real-world process, such as testing a new aircraft design or evaluating a new protein, such active methods can be very expensive. On the other hand, in many cases there is considerable prior data -- existing aircraft and protein designs, and advertisements and user click rates, etc. -- that could be leveraged to solve the optimization problem.

In this work, our goal is to develop an optimization approach to solve such optimization problems that can (1) readily operate on high-dimensional inputs comprising a narrow, low-dimensional manifold in the input space, (2) readily utilize offline static data, and (3) learn with minimal active data collection if needed. We can define this problem setting formally as the optimization problem
\begin{equation}
    \x^\star = \arg\max_{\x} f(\x), \label{eq:optimization}
\end{equation}
where the function $f(\x)$ is unknown, and we have access to a dataset $\data = \{ (\x_1, y_1), \dots, (\x_N, y_N) \}$, where $y_i$ denotes the value $f(\x_i)$. If no further data collection is possible, we call this data-driven model-based optimization, else we refer to it as active model-based optimization. This can also be extended to the \textit{contextual} setting, where the aim is to optimize the expected score function across a context distribution. That is,
\begin{equation}
    \pi^\star = \arg\max_{\pi} \expec_{c \sim p(\cdot)} [f(c, \pi(c))], \label{eq:contextual_optimization}
\end{equation}
where $\pi^\star$ maps contexts $c$ to inputs $\x$, such that the expected score under the context distribution $p(c)$ is optimized. As before, $f(c, \x)$ is unknown, and we use a dataset $\data = \{ (c_i, \x_i, y_i) \}_{i=1}^N$, where $y_i$ is the value of $f(c_i, \x_i)$. Such contextual problems with logged datasets have been studied in the context of contextual bandits~\citep{swaminathan2015counterfactual, joachims2018deep}.

A simple way to approach these model-based optimization problems is to train a proxy function ${f}_\theta(\x)$ or ${f}_\theta(c, \x)$, with parameters $\theta$, to approximate the true score, using the dataset $\data$. However, directly using ${f}_\theta(\x)$ in place of the true function $f(\x)$ in Equation~(\ref{eq:optimization}) generally works poorly, because the optimizer will quickly find an input $\x$ for which ${f}_\theta(\x)$ outputs an erroneously large value. This issue is especially severe when the inputs $\x$ lie on a narrow manifold in a high-dimensional space, such as the set of natural images~\citep{zhu2016generative}. The function ${f}_\theta(\x)$ is only valid near the training distribution, and can output erroneously large values when queried at points chosen by the optimizer. Prior work has sought to addresses this issue by using uncertainty estimation and Bayesian models~\citep{snoek15scalable} for ${f}_\theta(\x)$, as well as active data collection~\citep{snoek2012practical}. However, explicit uncertainty estimation is difficult when the function ${f}_\theta(\x)$ is very complex or when $\x$ is high-dimensional.

Instead of learning ${f}_\theta(\x)$, we propose to learn the inverse function, mapping from values $y$ to corresponding inputs $\x$. This inverse mapping is one-to-many, and therefore requires a \emph{stochastic} mapping, which we can express as $\finv_\theta(y,\z) \rightarrow \x$, where $\z$ is a random variable. We term such models \emph{model inversion networks} (MINs). 
MINs can handle high-dimensional input spaces such as images, can tackle contextual problems, and can accommodate both static datasets and active data collection. We discuss how to design active data collection methods for MINs, leverage advances in deep generative modeling~\citep{goodfellow2014generative,brock2018large}, and scale to very high-dimensional input spaces.
We experimentally demonstrate MINs in a range of settings, showing that they outperform prior methods on high-dimensional input spaces, perform competitively to Bayesian optimization methods on tasks with active data collection and lower-dimensional inputs, and substantially outperform prior methods on contextual bandit optimization from logged data~\citep{swaminathan2015counterfactual}.

==> Model inversion networks (MINs)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\rulesep}{\unskip\ \hrule\ }

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Model inversion networks (MINs)/method.tex <==
\section{Model Inversion Networks}
Here, we describe our model inversion networks (MINs) method, which can perform both active and passive model-based optimization over high-dimensional inputs.

\textbf{Problem statement.} Our goal is to solve optimization problems of the form $\x^\star = \arg\max_{\x} f(\x)$, where the function $f(\x)$ is not known, but we must instead use a dataset of input-output tuples $\data = \{(\x_i, y_i)\}$. In the contextual setting described in Equation~(\ref{eq:contextual_optimization}), each datapoint is also associated with a context $c_i$. For clarity, we present our method in the non-contextual setting, but the contextual setting can be derived analogously by conditioning all learned models on the context. In the \emph{active} setting, which is most often studied in prior work, the algorithm can query $f(\x)$ one or more times on each iteration to augment the dataset, while in the \emph{static} or \emph{data-driven} setting, only an initial static dataset is available. The goal is to obtain the best possible $\x^\star$ (i.e., the one with highest possible value of $f(\x^\star)$).

One na\"{i}ve way of solving MBO problems is to learn a proxy score function ${f}_\theta(\x)$ via empirical risk minimization, and then maximize it with respect to $\x$. However, na\"{i}ve applications of such a method would fail for two reasons. First, the proxy function ${f}_\theta(\x)$ may not be accurate outside the distribution on which it is trained, and optimization with respect to it may simply lead to values of $\x$ for which ${f}_\theta(\x)$ makes the largest mistake. The second problem is more subtle. When $\x$ lies on a narrow manifold in a very high-dimensional space, such as the space of natural images, the optimizer can produce invalid values of $\x$, which result in arbitrary outputs when fed into ${f}_\theta(\x)$. Since the shape of this manifold is unknown, it is difficult to constrain the optimizer to prevent this. This second problem is rarely addressed or discussed in prior work, which typically focuses on optimization over low-dimensional and compact domains with known bounds.  

\subsection{Optimization via Inverse Maps}
Part of the reason for the brittleness of the na\"{i}ve approach above is that ${f}_\theta(\x)$ has a high-dimensional input space, making it easy for the optimizer to find inputs $\x$ for which the proxy function produces an unreasonable output. Can we instead learn a function with a small input space, which implicitly understands the space of valid, in-distribution values for $\x$?
The main idea behind our approach is to model an inverse map  that produces a value of $\x$ given a score value $y$, given by $\finv_\theta : \mathcal{Y} \rightarrow \mathcal{X}$. The input to the inverse map is a scalar, making it comparatively easy to constrain to valid values, and by directly generating the inputs $\x$, an approximation to the inverse function must implicitly understand which input values are valid. As multiple $\x$ values can correspond to the same $y$, we design $\finv_\theta$ as a stochastic map that maps a score value along with a $d_z$-dimensional random vector to a $\x$, $\finv_\theta : \mathcal{Y} \times \mathcal{Z} \rightarrow \mathcal{X}$, where $\z$ is distributed according to a prior distribution $p_0(\z)$. 

The inverse map training objective corresponds to standard distribution matching, analogously to standard generative models, which we will express in a somewhat more general way to simplify the exposition later. Let $p_\data(\x, y)$ denote the data distribution, such that $p_\data(y)$ is the marginal over $y$, and let $p(y)$ be an any distribution on $\mathcal{Y}$, which could be equal to $p_\data(y)$. We can train the proxy inverse map $\finv_\theta$ by minimizing the following objective:
\begin{equation}
    \label{obj:basic}
    \loss_p(\data) = \expec_{y \sim p(y)} \left[ D \left(p_\data(\x|y), p_{\finv_\theta}(\x|y) \right) \right],
\end{equation}
where $p_{\finv_\theta}(\x|y)$ is obtained by marginalizing over $\z$, %$p_{\finv_\theta}(\x|y) = \int_{\z} p(\z) \cdot \mathbf{1}[[{\x = \finv_\theta(\z, y)}]] d\z$,
and $D$ is a measure of divergence between the two distributions. Using the Kullback-Leibler divergence leads to maximum likelihood learning, while Jensen-Shannon divergence motivates a GAN-style training objective. MINs can be adapted to the contextual setting by passing in the context as an input and learning $\finv_\theta(y_i, z, c_i)$.

{While the basic idea behind MINs is simple, a number of implementation choices are important for good performance. Instead of choosing $p(y)$ to be $p_\data(y)$, as in standard ERM, in Section~\ref{sec:reweighting} we show that a careful choice of $p(y)$ leads to better performance. In Section~\ref{sec:exploration}, we then describe a method to perform active data sampling with MINs. We also present a method to generate the best optimization output $\x^\star$ from a trained inverse map $\finv_\theta(\cdot, \cdot)$ during evaluation in Section~\ref{sec:inference}. The structure of the full MIN algorithm is shown in Algorithm~\ref{alg:cn_meta_alg}, and a schematic flowchart of the procedure is shown in Figure~\ref{fig:min_flowchart}.}   
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{images/mins_schematic_final.png}
    \caption{Schematic for MIN training and optimization. Reweighting (Section~\ref{sec:reweighting}) and, optionally, active data collection (Section ~\ref{sec:exploration}) are used during training. The MIN is then used to obtain the optimal input $\x^\star$ using the Approx-Infer procedure in Section~\ref{sec:inference}.}
    \label{fig:min_flowchart}
\end{figure}

\begin{algorithm}
\caption{Generic Algorithm for MINs}
\begin{algorithmic}[1]
  %\STATE Input: $p_\data(y)$: distribution of $y$ in $\data$ 
  \STATE Train inverse map $\finv_\theta : \mathcal{Y} \times \mathcal{Z} \rightarrow \mathcal{X}$ with Equation~(\ref{obj:basic})\!\!\!
  \STATE (optionally) perform active data collection
  \STATE return $\x^\star \leftarrow$ \textsc{Approx-Infer} ($\finv_\theta$, $p_\data(y)$)
\end{algorithmic}
\label{alg:cn_meta_alg}
\end{algorithm}

\subsection{Inference with Inverse Maps (Approx-Infer)}
\label{sec:inference}
Once the inverse map is trained, the goal of our algorithm is to generate the best possible $\x^\star$, which will maximize the true score function as well as possible. Since a score $y$ needs to be provided as input to the inverse map, we must select for which score $y$ to query the inverse map to obtain a near-optimal $\x$.
One na\"{i}ve heuristic is to pick the best $y_{\max} \in \data$ and produce $\x_{\max} \sim \finv_\theta(y^*_{\max})$ as the output. However, the method should be able to extrapolate beyond the best score seen in the dataset, especially in contextual settings, where a good score may not have been observed for all contexts.

In order to extrapolate as far as possible, while still staying on the valid data manifold, we need to measure the validity of the generated values of $\x$. One way to do this is to measure the agreement between the learned inverse map and an independently trained forward model ${f}_\theta$: the values of $y$ for which the generated samples $\x$ are predicted to have a score similar to $y$ are likely in-distribution, whereas those where the forward model predicts a very different score may be too far outside the training distribution. {This amounts to using the agreement between independently trained forward and inverse maps to quantify the degree to which a particular score $y$ is out-of-distribution.} Since the latent variable $z$ captures the multiple possible outputs of the one-to-many inverse map, we can further optimize over $z$ for a given $y$ to find the best, most trustworthy $\x$ subject to the constraint that $\z$ has a high likelihood under the prior. This can be formalized as the following optimization:
\begin{multline}
    \yquery, \zquery := \arg \max_{y, z} {f}_\theta(\finv_\theta(z, y))  \\
    \text{~~s.t.~~}  \vert\vert y - {f}_\theta(\finv_\theta(z, y)) \vert\vert_2 \leq \epsilon_1\\
    \log p_0(z) \geq \epsilon_2 
    \vspace{-70pt}
    \label{eqn:inference}
\end{multline}
This optimization can be motivated as finding an extrapolated score, higher than the observed dataset $\data$, that corresponds to values of $\x$ that lie on the valid input manifold, and for which independently trained forward and inverse maps agree.
Although this optimization uses an approximate forward map ${f}_\theta(\x)$, we show in our experiments in Section \ref{sec:experiments} that it produces substantially better results than optimizing with respect to a forward model alone. The inverse map substantially constraints the search space, requiring an optimization over a 1-dimensional $y$ and a (relatively) low-dimensional $z$, rather than the full space of inputs. {This can be viewed as a special (deterministic) case of a probabilistic optimization procedure, which we describe in Appendix~\ref{app:inference}.} 
\vspace{-5pt}
\subsection{Reweighting the Training Distribution}
\label{sec:reweighting}
A na\"{i}ve implementation of the training objective in Equation~(\ref{obj:basic}) samples $y$ from the data distribution $p_\data(y)$. However, as we are most interested in the inverse map's predictions for \emph{high} values of $y$, it is much less important for the inverse map to predict accurate $\x$ values for values of $y$ that are far from the optimum. We could consider increasing the weights on points with larger values of $y$. In the extreme case, we could train only on the best points -- either the single datapoint with the largest $y$ or, in the contextual case, the points with the largest $y$ for each context. {To formalize this notion,} we can define the \emph{optimal} $y$ distribution $p^*(y)$, which is simply the delta function centered on the best $y$, $p^*(y) = \delta_{y*}(y)$ in the deterministic case. If we assume that the observed scores have additive noise (i.e., we observe $f(\x) + \varepsilon, \varepsilon \sim \mathcal{N}$), then $p^*(y)$ would be a distribution centered around the optimal $y$.

{We could attempt to train only on $p^\star(y)$, as $y$ values far from optimum are much less important. However, this is typically impractical, since $p^\star(y)$ heavily down-weights most of the training data, leading to a very high-variance training objective.} We can instead choose $p(y)$ to trade off the variance due to an overly peaked training distribution and the bias due to training on the ``wrong'' distribution (i.e., anything other than $p^*(y)$).

When training under a distribution $p(y)$ other than $p_\data(y)$, we can use importance sampling, where we sample from $p_\data$ and assign an importance weight $\w_i = \frac{p(y_i)}{p_{\data}(y_i)},$ to each datapoint $(\x_i, y_i)$.
The reweighted objective is given by $\hat{\loss}_p(\data) := \frac{1}{|\data|} \sum_i \w_i \cdot \hat{D}(\x_i, \finv_\theta(y_i))$. 
By bounding the variance and the bias of the gradient of $\hat{\loss}_p(\data)$,
we obtain the following result, with the proof given in Appendix~\ref{app:bias_var}:

\begin{theorem}[Bias + variance bound in MINs]
\label{thm:grad_bias_variance}
Let $\loss{(p^*)}$ be the objective under $p^*(y)$ without sampling error: $\loss{(p^*)} = \expec_{y \sim p^*(y)}[D(p(\x|y), \finv(y))]$.
Let $N_y$ be the number of datapoints with the particular $y$ value observed in $\data$, 
% $N_y = \#\{(\x_i, y_i) \in \data ~|~ y_i = y \}$. 
For some constants $C_1, C_2, C_3$, with high confidence,
\begin{multline*}
    \expec\left[\vert\vert \nabla_\theta \hat{\loss}_p(\data) - \nabla_{\theta} \loss(p^*) \vert\vert_2^2\right] \leq C_1 \expec_{y \sim p(y)} \left[\frac{1}{N_y}\right] +\\
    C_2 \frac{d_2(p||p_\data)}{|\data|} + C_3 \cdot D_{\mathrm{TV}} (p^*, p)^2
\end{multline*}
where $d_2$ is the exponentiated Renyi divergence.
\vspace{-10pt}
\end{theorem}
Theorem~\ref{thm:grad_bias_variance} suggests a tradeoff between being close to the optimal distribution $p^*(y)$ (third term) and reducing variance by covering the full data distribution $p_\data$ (second term).
The distribution $p(y)$ that minimizes the bound in Theorem~\ref{thm:grad_bias_variance} has the following form: $p(y) \propto \frac{{N_y}}{N_y + K} \cdot g(p^*(y))$, where $g(p^*)$ is a monotonically increasing function of $p^*(y)$ that ensures that the distributions $p$ and $p^*$ are close.
We empirically choose an exponential parameteric form for this function $g$, which we describe in Section~\ref{sec:implementation}.
This upweights the samples with higher scores, reduces the weight on \emph{rare} $y$-values (i.e., those with low $N_y$), while preventing the weight on \emph{common} $y$-values from growing, since $\frac{N_y}{N_y + K}$ saturates to $1$ for large $N_y$. This is consistent with our intuition: we would like to upweight datapoints with high $y$-values, provided the number of samples at those values is not too low. For continuous-valued scores, we rarely see the same score twice, so we bin the $y$-values into discrete bins for the purpose of reweighting, as we discuss in Section~\ref{sec:implementation}.

\subsection{Active Data Collection via Randomized Labeling}
\label{sec:exploration}
% \vspace{-5pt}
While the passive setting requires care in finding the best value of $y$ for the inverse map, the active setting presents a different challenge: choosing a new query point $\x$ at each iteration to augment the dataset $\data$ and make it possible to find the best possible optimum.
Prior work on bandits and Bayesian optimization often uses Thompson sampling (TS)~\citep{russo2016information,russo2018tutorialthompson,Srinivas2010gaussian} as the data-collection strategy. TS maintains a posterior distribution over functions $p({f}_t|\data_{1:t})$. At each iteration, it samples a function from this distribution and queries the point $\x^\star_t$ that greedily minimizes this function. TS offers an appealing query mechanism, since it achieves sub-linear Bayesian regret (the expected cumulative difference between the value of the optimal input and the selected input), given by $\bigO(\sqrt{T})$, where $T$ is the number of queries.
Maintaining a posterior over high-dimensional parametric functions is generally intractable. However, we can approximate Thompson sampling with MINs. First, note that
sampling ${f}_t$ from the posterior is equivalent to sampling $(\x, y)$ pairs consistent with ${f}_t$ -- given sufficiently many $(\x, y)$ pairs, there is a unique smooth function ${f}_t$ that satisfies $y_i = {f}_t(\x_i)$. For example, we can infer a quadratic function exactly from three points. For a more formal description, we refer readers to the notion of eluder dimension~\citep{russo13eluder}. Thus, instead of maintaining intractable beliefs over the function, we can identify a function by the samples it generates, and define a way to sample synthetic $(\x, y)$ points such that they implicitly define a unique function sample from the posterior.

To apply this idea to MINs, we train the inverse map $\finv_{\theta_t}$ at each iteration $t$ with an \textit{augmented} dataset $\data'_{t} = \data_t \cup \mathcal{S}_t$, where $\mathcal{S}_t = \{ (\tilde{\x}_j, \tilde{y}_j) \}_{j=1}^K$ is a dataset of synthetically generated input-score pairs corresponding to unseen $y$ values in $\data_t$.
Training $\finv_{\theta_t}$ on $\data'_t$ corresponds to training $\finv_{\theta_t}$ to be an approximate inverse map for a function ${f}_t$ sampled from $p({f}_t|\data_{1:t})$, as the synthetically generated samples $\mathcal{S}_t$ implicitly induce a model of ${f}_t$. We can then approximate Thompson sampling by obtaining $\x^\star_t$ from $\finv_{\theta_t}$, labeling it via the true function, and adding it to $\data_t$ to produce $\data_{t+1}$. Pseudocode for this method, which we call ``randomized labeling,'' is presented in Algorithm \ref{alg:cn_practice}. In Appendix~\ref{app:regret_bound}, we further derive $\bigO(\sqrt{T})$ regret guarantees under mild assumptions. Implementation-wise, this method is simple, does not require estimating explicit uncertainty, and works with arbitrary function classes, including deep neural networks.

\vspace{-5pt}
\begin{algorithm}
\small
\caption{Active Data Collection with Model Inversion Networks via Randomized Labeling}
\label{alg:cn_practice}
\begin{algorithmic}[1]
    \STATE Initialize inverse map, $\finv_\theta: \mathcal{Y} \times \mathcal{Z} \rightarrow \inputspace$, dataset $\data_0 = \{\}$, 
    \FOR{step $t$ in \{0, \dots, T-1\}}
        \STATE Sample synthetic samples $\mathcal{S}_t = \{ (\x_i, y_i) \}_{i=1}^K$ corresponding to unseen data points $y_i$ (by randomly pairing noisy observed $\x_i$ values with unobserved $y$ values.)
        \STATE Train \textit{inverse map} $\finv_t$ 
        on $\data'_t = \data_t \cup \mathcal{S}_t$, using reweighting described in Section \ref{sec:reweighting}.
        \STATE Query function $f$ at $\x_t = \finv_t(\max_{\data'_t} y)$
        \STATE Observe outcome: $(\x_t, f(\x_t))$ and update $\data_{t+1} = \data_t \cup (\x_t, f(\x_t))$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Practical Implementation of MINs}
\label{sec:implementation}

In this section, we describe our instantiation of MINs for high-dimensional inputs with deep neural network models. GANs~\citep{goodfellow2014generative} have been successfully used to model the manifold of high-dimensional inputs, without the need for explicit density modelling and are known to produce more realistic samples than other models such as VAEs~\citep{kingma2013autoencoding} or Flows~\citep{dinh2016density}. The inverse map in MINs needs to model the manifold of valid $\x$ thus making GANs a suitable choice. We can instantiate our inverse map with a GAN by choosing $D$ in Equation~\ref{obj:basic} to be the \textit{Jensen-Shannon} divergence measure. Since we generate $\x$ conditioned on $y$, the discriminator is parameterized as $\disc(\x|y)$, and trained to output 1 for a valid $(\x, y)$ pair (i.e., where $y = f(\x)$ and $\x$ comes from the data) and 0 otherwise. Thus, we optimize the following objective:
\begin{multline*}
    \min_{\theta} \max_{\disc} \loss_p(\data) = \expec_{y \sim p(y)} \big[ \expec_{\x \sim p_\data(\x|y)}[\log \disc(x|y)] +\\ \expec_{\z \sim p_0(\z)} [\log (1 - \disc(\finv_\theta(\z, y)|y)] \big] 
\end{multline*}
This model is similar to a conditional GAN (cGAN), which has been used in the context of modeling distribution of $\x$ conditioned on a discrete-valued label~\citep{mirza2014conditional}.
As discussed in Section~\ref{sec:reweighting}, we additionally reweight the data distribution using importance sampling. To that end, we discretize the space $\mathcal{Y}$ into $B$ discrete bins $b_1, \cdots, b_B$ and, following Section~\ref{sec:reweighting}, weight each bin $b_i$ according to $p(b_i) \propto \frac{{N_{b_i}}}{N_{b_i} + \lambda} \exp\left(\frac{|{b_i} - y^*|}{\tau}\right)$, where $N_{b_i}$ is the number of datapoints in the bin, {$y^*$ is the maximum score observed}, and $\tau$ is a hyperparameter. {(After discretization, using notation from Section~\ref{sec:reweighting}, for any $y$ that lies in bin $b$, $p^*(y) := p^*(b) = \exp\left(\frac{|{b} - y^*|}{\tau}\right)$ and $p(y) := p(b) \propto \frac{{N_{b}}}{N_{b} + \lambda} \exp\left(\frac{|{b} - y^*|}{\tau}\right)$.)} Experimental details are provided in {Appendix C.4}. 

In the active setting, we perform active data collection using the randomized labelling algorithm described in Section~\ref{sec:exploration}.  In practice, we train two copies of $\finv_\theta$. The first, which we call the exploration model $\finv_{\text{expl}}$, is trained with data augmented via synthetically generated samples (i.e., $\data'_t$). The other copy, called the exploitation model $\finv_{\text{exploit}}$, is trained on only real samples (i.e., $\data_t$). This improves stability during training, while still performing data collection as dictated by Algorithm~\ref{alg:cn_practice}. {To generate the augmented dataset $\data'_t$ in practice, we sample $y$ values from $p^*(y)$ (the distribution over high-scoring $y$s observed in $\data_t$), and add positive-valued noise, thus making the augmented $y$ values higher than those in the dataset which promotes exploration. The corresponding inputs $x$ are simply sampled from the dataset $\data_t$ or uniformly sampled from the bounded input domain when provided in the problem statement. (for example, benchmark function optimization)}
After training, we infer best possible $\x^\star$ from the trained model using the inference procedure described in Section~\ref{sec:inference}. In the active setting, the inference procedure is applied on $\finv_{\text{exploit}}$, the inverse map which is trained only on real data points.  


==> Model inversion networks (MINs)/related.tex <==
\section{Related Work}

% Bayesian optimization 
\textbf{Bayesian and model-based optimization.} Most prior work on model-based optimization has focused on the active setting. This includes algorithms such as the cross entropy method (CEM) and related derivative-free methods~\cite{rubinstein96optimizationof, rubinstein2004cross}, reward weighted regression~\cite{peters2012reinforcement}, Bayesian optimization methods based on Gaussian processes~\cite{shahriari2016TakingTH, snoek2012practical,snoek15scalable}, and variants that replace GPs with parametric acquisition function approximators, such as Bayesian neural networks~\citep{snoek15scalable} and latent variable models~\citep{kim2018attentive,garnelo18neural,garnelo18conditional}, as well as more recent methods such as CbAS~\citep{brookes19a}. These methods require the ability to query the true function $f(\x)$ at each iteration to iteratively arrive at a near-optimal solution. We show in Section~\ref{sec:reweighting} that MINs can be applied to such an active setting as well, and in our experiments we show that MINs can perform competitively with these prior methods. Additionally, we show that MINs can be applied to the static setting, where these prior methods are not applicable. Furthermore, most conventional BO methods do not scale favourably to high-dimensional input spaces, such as images, while MINs can handle image inputs effectively.


\textbf{Contextual bandits.} Equation~\ref{eq:contextual_optimization} describes contextual bandit problems. Prior work on batch contextual bandits has focused on batch learning from bandit feedback (BLBF), where the learner needs to produce the best possible policy that optimizes the score function from logged experience. Existing approaches build on the counterfactual risk minimization (CRM) principle~\citep{swaminathan2015counterfactual,swaminathan2015selfnormalized},
and have been extended to work with deep nets~\citep{joachims2018deep}.
In our comparisons, we find that MINs substantially outperform these prior methods in the batch contextual bandit setting.

\textbf{Deep generative modeling.} Recently, deep generative modeling approaches have been very successful at modelling high-dimensional manifolds such as natural images~\citep{goodfellow2014generative,oord2016pixelrnn,dinh2016density}, speech~\citep{oord2018parallel}, text~\citep{yu2017seqgan}, alloy composition prediction~\citep{ngyuen_rebuttal}, and other data. {Unlike inverse map design, MINs solve an easier problem by learning the inverse map accurately only on selectively chosen datapoints, which is sufficient for optimization.} MINs combine the strength of such generative models with important algorithmic choices to solve model-based optimization problems. In our experimental evaluation, we show that these design decisions are important for adapting deep generative models to model-based optimization, and it is difficult to perform effective optimization without them. 


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\rulesep}{\unskip\ \hrule\ }

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

